On sampling determinantal and Pfaffian point processes on a quantum computer

DPPs were introduced by Macchi as a model in quantum optics the 1970s. Since then, they have been widely used as models and subsampling tools in statistics and computer science. Most applications require sampling from a DPP, and given their quantum origin, it is natural to wonder whether sampling a DPP on a quantum computer is easier than on a classical one. We focus here on DPPs over a finite state space, which are distributions over the subsets of $\{1,\dots,N\}$ parametrized by an $N\times N$ Hermitian kernel matrix. Vanilla sampling consists in two steps, of respective costs $\mathcal{O}(N^3)$ and $\mathcal{O}(Nr^2)$ operations on a classical computer, where $r$ is the rank of the kernel matrix. A large first part of the current paper consists in explaining why the state-of-the-art in quantum simulation of fermionic systems already yields quantum DPP sampling algorithms. We then modify existing quantum circuits, and discuss their insertion in a full DPP sampling pipeline that starts from practical kernel specifications. The bottom line is that, with $P$ (classical) parallel processors, we can divide the preprocessing cost by $P$ and build a quantum circuit with $\mathcal{O}(Nr)$ gates that sample a given DPP, with depth varying from $\mathcal{O}(N)$ to $\mathcal{O}(r\log N)$ depending on qubit-communication constraints on the target machine. We also connect existing work on the simulation of superconductors to Pfaffian point processes, which generalize DPPs and would be a natural addition to the machine learner's toolbox. In particular, we describe "projective" Pfaffian point processes, the cardinality of which has constant parity, almost surely. Finally, the circuits are empirically validated on a classical simulator and on 5-qubit IBM machines.

==> applications.tex <==
\subsection{Uniform spanning trees and related DPPs}

\subsection{Column subset selection}
\cite{BeBaCh20b} propose to select the columns of a ``fat" matrix\footnote{Note our different notation compared to \citep{BeBaCh20b}, who use $N$ for the number of rows.} $\bX \in\mathbb{R}^{n\times N}$, $N\gg n$, using the projection DPP with rank-$k$ kernel 
\begin{equation}
    \label{e:ayoub_kernel}
    \bK = \bV_{:,1:k}\bV_{:,1:k}^T,
\end{equation}
where $\bX = \bU \mathbf{\Sigma} \bV^T$ is the SVD of $\bX$. 
The authors prove in particular that the resulting random subset of $k$ indices in $\{1, \dots, N\}$ can be advantageously used to select columns of $\bX$ (i.e., features) in sketched linear regression.
The only downside of such a method is the cost of sampling the DPP on a classical computer, the bottleneck of which is the $\cO(Nk^2)$ cost of performing $k$-SVD. 
Once the decomposition \eqref{e:ayoub_kernel} is known, vanilla DPP sampling \citep{HKPV06} costs $\cO(Nk^2)$ as well, and the randomized version of \cite{BTA22} further takes the cost down in expectation to $\cO(Nk + k^3\log k)$.

We now show how to build a quantum circuit of depth $N$ that approximately samples from the corresponding DPP. 
Exact sampling as in Section~\ref{s:circuit_for_projection_DPPs} requires to have the decomposition \eqref{e:ayoub_kernel} at hand, while we want to avoid the cost of obtaining $\cO(\bV_{:,1:k})$. 
We thus propose to use the circuit for Gaussian density matrices from Section~\ref{s:circuit_for_Gaussian_rho} with $\tilde \bK \propto \bX^T\bX$, and take the temperature to zero in order to approximately sample from the DPP with kernel \eqref{e:ayoub}.


